Split Optimization for Protein/Ligand Binding Models

In this paper, we investigate potential biases in datasets used to make drug binding predictions using machine learning. We investigate a recently published metric called the Asymmetric Validation Embedding (AVE) bias which is used to quantify this bias and detect overfitting. We compare it to a slightly revised version and introduce a new weighted metric. We find that the new metrics allow to quantify overfitting while not overly limiting training data and produce models with greater predictive value.

==> sections/stuff.tex <==

\subsection{Notes}
\begin{itemize}
\item Atomwise uses different $n$ values in paper and computation
\item Atomwise truncates data at 10,000 molecules (probably so that they can fit distance matrix in memory)
\item use of default settings and num estimators 100 leads to memorization of training set, and so is prone to exaggerate the effect of bias on performance.
\end{itemize}


\section{Score optimization evaluation}
Assume that, for a fixed target protein, Validation Embedding (VE) scores are roughly distributed normally. Then the cumulative distribution function (see, e.g., \cite{statsReference}) $F(\epsilon)$ gives an estimate for the probability that a given score sample will have value less than $\epsilon$. The inverse of $F(\epsilon)$ is the number of samples to be drawn from the distribution so that the expected number of samples with value less than $\epsilon$ is equal to one. This suggests a naive stochastic optimization strategy for minimizing the score:
\begin{algorithm}[Naive stochastic score optimization]
Given binary labeled metric data and a score goal $\epsilon$:

\begin{enumerate}
    \item Sample the score and approximate $F(\epsilon)$.
    \item If a sample with score less than $\epsilon$ has not yet been found, then compute the required sample size $N=1/F(\epsilon)$.
    \item If $N$ is less than the number of samples already drawn, then use the minimum score split already produced. Otherwise, sample $N$ times and take the minimum score split.
\end{enumerate} 
\end{algorithm}
This strategy is clearly inefficient if $N$ is very large, i.e., if the $z$-score of $\epsilon$ is far from zero. It may therefore serve as a sanity check on other forms of optimization. If an optimization method is not outperforming this stochastic method, it should be stopped: either because it is not working or else is approaching a local minimum value of the score. Note that in the case of fingerprint similarity, the score is bound below by -2. We expect it to have a minimum strictly larger than that.

\begin{performance} 
Let $\smin$ be the minimum score score acheived during $t$ seconds of computation using optimization method $\O$. If the mean time to compute the score for this data set is $\mu$, then compute \[\perf_{\O}(t) = \frac{t}{\mu}\cdot F(\smin).\]
\end{performance}
The right hand side is the expected number of samples with score less than $\smin$ after having sampled $t/\mu$ times. If $\O$ is the naive stochastic optimizer, then $\perf_{\O}(t)$ should be be close to one, and become increasingly positive as $\smin$ approaches the minimum for the score of the dataset. Small values of $\perf_{\O}$ indicate that the optimizer $\O$ is outperforming the naive method, and increasing values over $t$ indicate that $\smin$ has reached a local minimum.

\subsection{Evidence of normality}
We use the new VE score, as it is more robust than AVE bias. Additional justification is presented in Section \ref{equivalenceSection}.

We accumulate the scores for all targets after normalizing by subtracting each target's mean and dividing by its standard deviation. The resulting aggregate histograms are presented in Figure \ref{aggDist}. We assume that the distribution is normal (red). {\bf{Comment about truncation effects.}}


\subsection{Splits}
We produce training/validation splits via Bournoulli process (P(training)=0.8), resulting in normally distributed split ratios with mean 0.8 and standard deviation 0.008. Using the 2$\sigma$-rule, we expect that 95\% of splits have ratio between 0.784 and 0.816. Sampling splits using a Bournoulli process yielded Pearson correlations between score and split size of 0.030, 0.003, 0.007 for dekois, MUV, and DUDE data sets, respectively. We use this as evidence that relaxing the split size constraint (due to stochastic generation) has negligible effect on statistical analysis of score. 

\begin{figure}[h]
\begin{minipage}{0.3\textwidth}
\includegraphics[scale=0.4]{MUVaggScores.png}
\end{minipage}
\begin{minipage}{0.3\textwidth}
\includegraphics[scale=0.4]{DUDEscoreAgg.png}
\end{minipage}
\begin{minipage}{0.3\textwidth}
\includegraphics[scale=0.4]{dekoisAggScores.png}
\end{minipage}
\caption{Aggregate score distributions by dataset}
\label{aggDist}
\end{figure}


\begin{table}[h]
\begin{tabular}{|c|c|c|c|c|c|c|}
     \hline Data set & Targets & Samples & Mean & Std & Min & Max  \\
     \hline dekois & 81 & 3.04e6&  0.476 & 0.184 & 0.153&0.866 \\
     \hline MUV & 16& 4.10e3& 0.144& 0.070& 0.040&0.288\\
     \hline DUDE &77& 3.49e5 & 0.977& 0.186&-0.21&0.063\\
     \hline
\end{tabular}
\caption{Statistics of the mean of the scores for each target (by dataset)}
\end{table}

\begin{table}[h]
\begin{tabular}{|c|c|c|c|c|}
     \hline Data set &  Mean & Std & Min & Max \\
     \hline dekois & 0.056 & 0.012 & 0.029 & 0.091 \\
     \hline MUV & 0.073& 0.016& 0.039 & 0.100 \\
     \hline DUDE & 0.028&0.008& 0.015& 0.100\\
     \hline
\end{tabular}
\caption{Statistics of the standard deviation of the scores for each target (by dataset)}
\end{table}

\section{AUC and VE score correlation}
We sample 20 splits from each target of each data set, standardize the VE and AUC scores, and aggregate. Perason correlation coefficients of 0.42, 0.45, and 0.30 are reported for dekois, MUV, and DUDE, respectively. See Figure \ref{aggCorr}.

\begin{figure}[h]
\begin{minipage}{0.3\textwidth}
\includegraphics[scale=0.4]{dekoisCorrelation.png}
\end{minipage}
\begin{minipage}{0.3\textwidth}
\includegraphics[scale=0.4]{MUVCorrelation.png}
\end{minipage}
\begin{minipage}{0.3\textwidth}
\includegraphics[scale=0.4]{DUDECorrelation.png}
\end{minipage}
\caption{Aggregate AUC vs VE scores by dataset}
\label{aggCorr}
\end{figure}

\begin{tabular}{|c|c|c|c|c|}
split score    &   AUC &    nnAUC   &     F1  &    nnF1\\
\hline
 1.000000 & 0.286901 & 0.650737 & 0.287238 & 0.582286\\
 0.286901 & 1.000000  & 0.379866  & 0.999995  & 0.330288\\
0.650737  & 0.379866  & 1.000000  & 0.379603  & 0.952910\\
 0.287238  & 0.999995 & 0.379603  & 1.000000  & 0.330019\\
 0.582286  & 0.330288  & 0.952910  & 0.330019  & 1.000000
\end{tabular}

\section{Comparison of VE score and AVE bias}\label{equivalenceSection} 
\input{bias_equivalence}
